Approximating LCS in Linear Time: Beating the $\sqrt{n}$ Barrier

Longest common subsequence (LCS) is one of the most fundamental problems in combinatorial optimization. Apart from theoretical importance, LCS has enormous applications in bioinformatics, revision control systems, and data comparison programs. Although a simple dynamic program computes LCS in quadratic time, it has been recently proven that the problem admits a conditional lower bound and may not be solved in truly subquadratic time. In addition to this, LCS is notoriously hard with respect to approximation algorithms. Apart from a trivial sampling technique that obtains a $n^{x}$ approximation solution in time $O(n^{2-2x})$ nothing else is known for LCS. This is in sharp contrast to its dual problem edit distance for which several linear time solutions are obtained in the past two decades.

==> BoundingMatchingPairs.tex <==
\section{Algorithm \ref{alg:6}: Bounding the Number of Matching Pairs}


%\begin{observation}
%	\label{obs:3}
%	If $R=O(n^{3/2-\epsilon})$, Algorithm \ref{alg:6} is an $O(n^{1/2-\epsilon})$ approximation for $\lcs$.
%\end{observation}

\begin{tcolorbox}
	In the instances which are not $O(n^{1/2-\epsilon})$-approximable with Algorithms \ref{alg:1}, \ref{alg:2}, and \ref{alg:6} we have:
	\begin{itemize}
		\item $m = \Omega( n^{1/2-\epsilon}).$
		\item $|\llcs(s,\bar s)| = \Omega( n^{1/2-\epsilon}).$
		\item $R = \Omega(n^{3/2-\epsilon})$
	\end{itemize}
\end{tcolorbox}




==> RandomShift.tex <==
\section{Algorithm \ref{alg:4}: Random Shift Algorithm}

 

\begin{tcolorbox}
	\textsf{Inputs:} $s,\sbar$.\\
	\textsf{Precondition}
	\begin{itemize}
		\item for each two randomly selected blocks $b_i$ and $\barblock_j$ of $s$ and $\sbar$, $$\mathbb{E}(|\llcs(b_i,\barblock_j)|) \geq n^\nu$$ 
	\end{itemize}
	\textsf{Approximation factor:} $O(n^{1/2-\nu})$
\end{tcolorbox}

%\begin{tcolorbox}
%	We can suppose w.l.o.g that in the instances which are not $O(n^{1/2-\epsilon})$-approximable with Algorithms \ref{alg:1}, \ref{alg:2},  \ref{alg:6}, and \ref{alg:7} we have:
%	\begin{itemize}
%		\item $m = \Omega( n^{1/2-\epsilon}).$
%		\item $|\llcs(s,\bar s)| = \Omega( n^{1/2-\epsilon}).$
%		\item $R = \Omega(n^{3/2-\epsilon})$
%		\item The frequency of each character $i$ in each of $s$ and $\bar{s}$ is $\Omega(n^{1/2-\epsilon})$.
%	\end{itemize}
%\end{tcolorbox}


==> Refinements.tex <==
\section{Refinement Algorithms}

\subsection{Removing Low Frequency Characters}
\begin{tcolorbox}
	%In the instances which are not $O(n^{1/2-\epsilon})$-approximable with Algorithm \ref{alg:1}, we have 
	\textsf{Inputs:} $s$ and $\bar{s}$.\\
	\textsf{Precondition}
	\begin{itemize}
		\item $|\llcs(s,\sbar)| = \Omega(n^{1-\gamma})$ 		
		\item The solution of Algorithm \ref{alg:7} is not a $1/2+\gamma $-approximation.
	\end{itemize}
	\textsf{Guarantee:} 
	\begin{itemize}
	\item Each character in $s$ and $\sbar$ has frequency $\Omega(n^{1/2-\gamma})$
	\item $|\llcs(s,\sbar)| = \Omega(n^{1-\gamma})$ 
	\end{itemize}	
\end{tcolorbox}

\subsection{Random Selection}
\begin{tcolorbox}
	%In the instances which are not $O(n^{1/2-\epsilon})$-approximable with Algorithm \ref{alg:1}, we have 
	\textsf{Inputs:} $s$ and $\bar{s}$.\\
	\textsf{Precondition}
	\begin{itemize}
	\item $|\flcs| = \Omega(n^{1-\delta})$
	\item $m= \Omega(n^{1/2+\eta})$
	\item The solution of Algorithm \ref{alg:3} is not  a $(1/2+\kappa)$-approximation. 
	\end{itemize}
	\textsf{Guarantee:} 
	\begin{itemize}
		\item	Both $s$ and $\sbar$ are semi-permutations.
		\item	$\mathbb{E}(|\flcs|) = \Omega(n^{1-\delta-\kappa})$.
		\item $m= \Omega(n^{1/2+\eta})$
	\end{itemize}
\end{tcolorbox}

\subsection{Refinement}
\begin{tcolorbox}
	%In the instances which are not $O(n^{1/2-\epsilon})$-approximable with Algorithm \ref{alg:1}, we have 
	\textsf{Inputs:} $s,\sbar$\\
	\textsf{Precondition}
	\begin{itemize}
		\item \textcolor{magenta}{Both $s$ and $\bar{s}$ are semi-permutations with parameter $\alpha$.}
		\item $m= \Omega(n^{1/2+\eta})$
		\item The solution of Algorithm \ref{alg:3} is not  a $(1/2+\kappa)$-approximation. 
	\end{itemize}
	\textsf{Guarantee:} 
	\begin{itemize}
		\item	Both $s$ and $\sbar$ are complete-permutations with parameter $??$.
		
	\end{itemize}
\end{tcolorbox}

==> SemitoFull.tex <==
\section{Converting Semi-permutations to Complete Permutations}



\begin{tcolorbox}
	\textsf{Inputs:} $s,\sbar$.\\
	\textsf{Precondition}
	\begin{itemize}
		\item both $s$ and $\sbar$ contain $\Omega(n^{1-\alpha})$ blocks
		\item Each block is a permutation of a subset of the characters in $\Sigma$. \item Each character character is appeared in a random block with probability $n^{-\beta}$ 
		\end{itemize}
		\textsf{Post Condition:} 
		\begin{itemize}
			\item Each block is updated based on $O(n^{\beta}\log n)$ other blocks  
		\end{itemize}
		\end{tcolorbox}


==> ideas.tex <==

\section{Ideas}\label{ideas}

Here we briefly discuss the current ideas for breaking the $\sqrt{n}$ barrier. We assume for simplicity that each character of $s$ and $\bar{s}$ is an integer number between $1$ and $1 \leq m \leq n$.

\begin{definition}
An instance of the $\lcs$ problem  is \emph{hard}, if it can not be approximated with factor $\bar{o}(\sqrt n )$ by the ideas in this section.
\end{definition}
 In this section, we propose three simple linear time solutions for \lcs\ that narrow down the hard instances to some very structured inputs.  

\begin{definition}
	Define $\tildbar$ to be a notation similar to $\tildorder$ except that $\tildbar$ ignores all $n^{o(1)}$ factors, i.e., $$f(n) \in \tildbar(g(n))  \iff  f(n) \in \tildorder(n^{o(1)}g(n)).$$
	$\omegabar, \bar{o},$ and  $\bar{\omega}$ are also defined the same way.
\end{definition}

\subsection{Counting the Characters}

We start with a simple observation: by Pigeonhole principle, there is a character in $\Sigma$ which is appeared at least $|\flcs|/m$ times in $\flcs$. Thus, the string that is consisted of the character with the maximum frequency in both $s$ and $\bar{s}$, is a  $m$-approximation of $\flcs$. Algorithm \ref{alg:1} is based upon this idea. In this algorithm, $C_1[i]$ and $C_2[i]$ refer to the frequency of character $i$ in $s$ and $\bar{s}$ respectively. The algorithm finds a character $i$ that maximizes $\min{(C_1[i],C_1[i])},$
and returns a string of length $\min{(C_1[i],C_1[i])}$ only consisting character $i$. 
\vspace{1cm}

\begin{algorithm}[H]
	\KwData{
		$s$ and $\bar{s}$.}
	\KwResult{An approximate solution for \lcs.}
	$C_1, C_2 \leftarrow$ two arrays of size $m$ initially set to $0$.\\
	\For{$i \in [1,n]$}{
		$C_1[s_i] \leftarrow C_1[s_i] + 1$\;
		$C_2[\bar{s}_i] \leftarrow C_2[\bar{s}_i] + 1$\;
	}
	$mx \leftarrow 0$\;
	\For{$i \in [1,m]$}{
		\If {$\min\{C_1[i], C_2[i]\}>mx$}{
			$mx = \min\{C_1[i], C_2[i]\}$ \;
			$idx = i$\;
		}
	}
	$r$ =  a string consisting $mx$ copies of character $idx$ \;	
	\textbf{Return}($r$)\;
	
	\caption{Count the characters}
	\label{alg:1}
\end{algorithm}

\begin{observation}[Restated]
	If $m = \bar{o}(\sqrt n)$, then Algorithm \ref{alg:1} is an $\bar{o}(\sqrt n)$-approximation algorithm for $\lcs$. Thus, in the hard instances $m=\omegabar(\sqrt{n})$.
\end{observation}



\subsection{Bounding the Solution Size}

In the next step, we show that the instances with small solution sizes can be $\bar{o}(\sqrt n)$-approximated in linear time. Consider two strings $s$ and $\bar{s}$ such that $\flcs = \tildbar(n^{1-\epsilon})$, where $\epsilon>0$ is a constant. We argue that for such an instance, Algorithm \ref{alg:2} returns an $\tildbar(n^{(1-\epsilon})/2)$-approximation solution. This algorithm has a structure very similar to Algorithm \ref{alg:5}: first, it samples a string $s^*$ with every symbol of $s$ being in $s^*$ with probability $n^{-(1-\epsilon)/2}$. Since every symbol of $\flcs$ is appeared in $s^*$ with probability $n^{-(1-\epsilon)/2}$, the expected size of $\llcs(s^*,\bar{s})$ is at least $$|\flcs| \cdot n^{-(1-\epsilon)/2},$$ which approximates $\flcs$ with a factor of $\tildbar(n^{(1-\epsilon)/2})$. The expected size of $s^*$ is $n^{(1+\epsilon)/2}$ and hence, using dynamic programming declared with Formula \eqref{dp2}, we can find $\llcs(s^*,\bar{s})$ in time $$\tildbar(n^{(1+\epsilon)/2} \cdot n^{(1-\epsilon)/2}) = \tildbar(n).$$  

\begin{observation}[Restated]\label{obs:2}
If the solution size is $\tildo(n)$, Algorithm \ref{alg:2} is an $\tildo(\sqrt n)$ approximation for $\lcs$. Thus, in the hard instances the size of the solution is $\omegabar(n)$.
\end{observation}

\begin{algorithm}[H]
	\KwData{
		$s$ and $\bar{s}$.}
	\KwResult{An approximate solution for \lcs.}
	$s^* \leftarrow $ an empty string\;
	\For{$i \in [1,n]$}{
		$p \leftarrow$ a random variable which is equal to $1$ with probability $n^{(\epsilon - 1)/2}$ and 0 otherwise.\;
		\If {$p = 1$}{
			add $s_i$ to the end of $s^*$\;
		}
	}
	The expected size of $s^*$ is  $n^{(1+\epsilon)/2}$. \\
	$DP \leftarrow$ A 2d array of size $|s^*| \times n^{(1-\epsilon)/2}$\;
	%Fill the array $DP$ with the following rule:
	%$DP[i][j] := $ the smallest index $k$ of $\bar{s}$ such that $$\mathsf{lcs}(s^*[1,i], \bar{s}[1,k]) \geq j$$\;
	%\textbf{Report}(the largest $j$ such that $DP[|s^*|][j] < \infty$)\;
	Compute $\llcs(s^*,\bar{s})$ using Formula \eqref{dp2}.
	\caption{Random Sampling}
	\label{alg:2}
\end{algorithm}

\subsection{Bounding Number of the Matching Pairs}

Let $R := |\{(i,j) | s_i = \bar{s}_j\}|$ be the number of matches in $s$ and $\bar{s}$. We show that if $R = \tildo(n^{3/2})$, then a near-linear time algorithm can $\tildo(\sqrt n)$-approximate $\flcs$. 
Apostolico and Guerra in ~\cite{hunt1977fast} give an $\tildorder(n+R)$ exact algorithm for solving $\lcs$. The basic idea behind their solution is as follows: let $M$ be an array of size $R$, where each element  in $M$ is a pair of indices that corresponds to a matching pair of $s$ and $\bar{s}$. In addition, suppose that the elements in $M$ are sorted according to the following rule:
\begin{equation}
\label{compare}
(i,j)<(i',j') \iff i<i' \mbox{ or } (i=i' \mbox{ and } j>j').
\end{equation}

It can be easily observed that finding $\flcs$ is equivalent to finding the longest subsequence of $M$ that is increasing in term of the second element of each pair, which can be found in $\tildorder(R)$. Based on their method, we propose an $\tildorder(n+R/\alpha)$ time algorithm with the approximation factor of $\alpha$. Let $M^*$ be an array where every pair in $M$ is in $M^*$ with probability $\alpha$. The expected size of $M^*$ is $R/\alpha$ and since each pair is appeared in $M^*$ with probability $\alpha$, the expected size of the longest increasing subsequence (as defined above) of $M^*$ is at least $\flcs/\alpha$ which approximate $\flcs$ with a factor of $\alpha$. 

We argue that we can construct $M^*$ in time $\tildbar(R/\alpha)$ from $s$ and $s'$. To do so, we iteratively sample the index of the next element of $M^*$ using a geometric distribution with parameter $\alpha$ which determines its distance to the currently selected index.  
 Next, for every sampled number $i$, we find the $i$'th matching pair of $M$. Note that to find the $i$'th matching pair, we don't need to explicitly access $M$; we can find it in time $O(\log n)$ using a simple handy data structure of size $O(n)$.


\vspace{0.5cm}
\begin{algorithm}[H]
	\KwData{
		$s$ and $\bar{s}$. $R$: number of matching pairs of $s$ and $s'$}
	\KwResult{An $\alpha$-approximate solution for \lcs.}
	$M^* = $ empty array \;
	$j \leftarrow 0$ \;
	$P =$ a geometric probability distribution on $\{1,2,\ldots\}$ with $P(Y = k) = (1-\alpha)^{k-1} \alpha$ \; 
	\While{$j<R$}{
		Sample $x$ from $P$ \;
		$j \leftarrow j+x$ \;
		\If{$j\leq R$}{
			Add the $j$'th element of $M$ to $M^*$ \;
		} 
	}
	Find the longest subsequence of $M^*$ which is increasing in term of the second element. 
\vspace{0.5cm}
\caption{Random Sampling 2}
\label{alg:6}
\end{algorithm}




\vspace{0.5cm}
Now, suppose that there exists a constant $\epsilon$, where $R = \tildbar(n^{3/2-\epsilon})$. By setting $\alpha = n^{1/2-\epsilon}$ we have an $n^{1/2-\epsilon}$ approximation algorithm with time $$\tildbar(n+ n^{3/2-\epsilon -1/2 + \epsilon}) = \tildbar(n).$$ 
 Hence, Observation \ref{obs:3} holds.

\begin{observation}[Restated]
	\label{obs:3}
	If $R=\tildo(n^{3/2})$, a linear time $\tildo(\sqrt n)$ approximation algorithm exists for $\lcs$. Hence, in the hard instances we have $R= \omegabar(n^{3/2})$.
\end{observation}

\subsection{Bounding the Frequency of each Character}
In this section, we give a lower-bound on the frequency of each character in $s$ and $\bar{s}$. Note that we already have an upper-bound: recall  in Algorithm \ref{alg:1}, if there exists a character $i$ such that $\min(C_1[i],C_2[i]) \notin \tildbar(\sqrt n),$ then Algorithm \ref{alg:1} returns a solution with approximation factor of $\tildo(\sqrt{n})$. As a consequence, Observation \ref{upperbound} holds.

\begin{observation}
	\label{upperbound}
	For every character $i$ we have $\min(C_1[i],C_2[i]) = \tildbar(\sqrt n)$.
\end{observation}

\begin{definition}
A character $i$ has a low frequency in string $r$, if the number of times that this character is appeared in $r$ is $\tildo(\sqrt{n})$. Otherwise, we say character $i$ has a high frequency in $r$. In addition, define $r_L$ and $r_H$ as the substrings of $r$ restricted to the characters with low and high frequency, respectively. 
\end{definition}

Now, consider $s_L,s_H,\bar{s}_L$, and $\bar{s}_H$. Since $s_L$ and $s_H$ cover $s$ and $\bar{s}_H$ and $\bar{s}_H$ cover $\bar{s}$, we have
\begin{equation}
\label{ineq:1}
  \llcs(s_L,\bar{s}_L) + \llcs(s_L,\bar{s}_H) + \llcs(s_H,\bar{s}_L) + \llcs(s_H,\bar{s}_H)\geq \flcs
\end{equation}
which means 
$$
 \max\{\llcs(s_L,\bar{s}_L) , \llcs(s_L,\bar{s}_H) , \llcs(s_H,\bar{s}_L) , \llcs(s_H,\bar{s}_H)\} \geq \flcs/4.
$$

Hence, solving $\lcs$ for all these four sub-instances and returning the maximum, yields a $4$-approximation solution to $\flcs$. Besides, if we $\bar{o}(\sqrt n)$ approximate these sub-instances and return the maximum, we have an $\bar{o}(\sqrt n)$ approximation of $\flcs$. Here we claim that in the first three sub-instances, number of the  matching pairs is $\tildo(n^{3/2})$, which means using Algorithm \ref{alg:6} we can $o(\sqrt n)$ approximate $\llcs(s_L, \bar{s}_L)$, $\llcs(s_L, \bar{s}_H)$, and $\llcs(s_H, \bar{s}_L)$ in linear time. 

\begin{lemma}
	Number of the matching pairs of $(s_L,\bar{s}_L), (s_L,\bar{s}_H) ,$ and  $(s_H,\bar{s}_L)$  is  $\tildo(n^{3/2})$.
\end{lemma}
\begin{proof}
	We prove the statement for $(s_L,\bar{s}_H)$, but the same proof can be applied to the other cases.
	
	Let $p_i$ be the frequency of the $i$'th symbol of $\bar{s}_H$ in $s_L$. Total number of matching pairs of
$s_L$ and $\bar{s}_H$ is $$\sum_{1 \leq i \leq |\bar{s}_H|} p_i.$$ Since $s_L$ contains only low frequency character, 
 $p_i = \tildo(\sqrt n)$. Furthermore, we have $|\bar{s}_H| \leq n$, which means
$$
\sum_{i \leq |s_L|} p_i \in \tildo(n^{3/2}).
$$
\end{proof}

Now, consider Algorithm \ref{alg:7}. This algorithm solves the first three sub-instances and returns the maximum. 

\begin{observation}
	Algorithm \ref{alg:7} guarantees an $\tildo(\sqrt n)$ approximation of $\flcs$, 
	if and only if $$\max\{\llcs(s_L,\bar{s}_L), \llcs(s_L,\bar{s}_H), \llcs(s_H,\bar{s}_L) \}= \omegabar(n).$$  Thus, in the hard instances
	$$\max\{\llcs(s_L,\bar{s}_L), \llcs(s_L,\bar{s}_H), \llcs(s_H,\bar{s}_L) \}= \tildo(n).$$
\end{observation}

Recall that by Observation \ref{obs:2} we know that in the hard instances, the solution size is $\omegabar(n)$.
This means that the contribution of the characters with low frequency is negligible in $\flcs$ and we can remove these characters without a considerable decrease in the solution size. 
 Therefore, Observation \ref{obs:5} holds.

\begin{observation}[Restated]
	\label{obs:5}
	We can assume w.l.o.g that in the hard instances, the frequency of each character is $\omegabar(\sqrt n)$ in both $s$ and $\bar{s}$.
\end{observation} 

As a consequence of Observation \ref{obs:5} we can say $|\Sigma| = m = \bar{\theta}(\sqrt n)$.  

\begin{algorithm}[H]
	\KwData{
		$s$ and $\bar{s}$.}
	\KwResult{An approximate solution for \lcs.}
	Construct $s_L,s_H,\bar{s}_L,\bar{s}_H$ \;
	Approximate $\llcs(s_L,\bar{s}_L)$, $\llcs(s_L,\bar{s}_H)$, and $\llcs(s_H,\bar{s}_L)$ using Algorithm \ref{alg:6} and return the maximum\;
	\caption{Low, High frequency algorithm}
	\label{alg:7}
\end{algorithm}

%Thus, to approximate $\flcs$ it only suffices to approximate the cases that both the strings contain only high frequency characters. 

%Note that the characters in $s_h$ and $\bar{s}_h$ have a frequency of $\theta(\sqrt{n})$. 
%Observation \ref{upperbound} provides an upper-bound on the frequency of number of times that each character is appeared in both the strings.   

%Therefore, Observation \ref{obs:4} holds.

%\begin{observation}
%	\label{obs:4}
%	In the hard instances we have $m = \theta(\sqrt{n})$. Also, every character contributes $\tildbar(\sqrt{n})$ to the solution and appears $\theta(\sqrt{n})$ times in both strings.
%\end{observation}


\subsection{Semi-permutations}
In this section, we propose a linear time approximation algorithm that narrows down the space of the hard instances to a very special structure, which we name it semi-permutations. Consider Algorithm \ref{alg:3}. This algorithm divides $s$ and $\bar{s}$ into $\sqrt n$ blocks of size $\sqrt n$. denote by $\block_i$ and $\barblock_i$, the $i$'th block of $s$ and $\bar{s}$, respectively. The algorithm constructs a $\sqrt{n} \times \sqrt{n}$ table $T$, 
%where $T[i][j]$ is determined as follows: we sample $10$ random locations of block $i$, and for each sample, we check the frequency of the character in that location in both $\block_i$ and $\barblock_j$. If the frequency of that character in both $\block_i$ and $\barblock_i$ was $\tildbar(n^\epsilon)$ we  
where $T[i][j]$ is the frequency of the character which appears most in $\block_i$ and $\barblock_j$. In fact, $T[i][j]$ approximates the length of  $\llcs(\block_i,\barblock_j)$ using Algorithm \ref{alg:1}. Note that we can fill table $T$ in  $\tildbar(n)^*$. 







With use of $T$, Algorithm \ref{alg:6} finds the longest common subsequence of $s$ and $\bar{s}$ with the following two constraints:

\begin{itemize}
	\item Characters selected from a block are similar.  
	\item Selected characters of a block in $s$ are mapped to characters in the same block in $\bar{s}$, and vice versa.
\end{itemize}

Denote by $\clcs(s,\bar{s})$, the longest common subsequence of $s$ and $\bar{s}$ with the constraints described above. We use dynamic programming to calculate $\clcs(s,\bar{s})$. Let $D$ be a $\sqrt{n} \times \sqrt{n}$ table where $D[i][j]$ stores the length of the longest restricted common subsequence of the first $i$ block of $s$ and the first $j$ block of $\bar{s}$. Then, $D[i][j]$ can be computed by the following recursive formula:
\begin{equation}
\label{eq:2}
D[i][j] = \begin{cases}
0 &i=0 \mbox{ or } j=0 \\
\max\{D[i][j-1],D[i-1][j], T[i][j]+ D[i-1][j-1]\} &i,j>0
\end{cases}
\end{equation}
Total running time of Algorithm \ref{alg:3} is $\tildbar(n)$. We now determine the conditions under which this algorithm returns an $\bar{o}(\sqrt{n})$ approximate solution.
\begin{definition}
We say a block is valuable if it contributes $\omegabar(\sqrt n)$ of its symbols to $\flcs$.
\end{definition} 

\begin{algorithm}[H]
	\KwData{
		$s$ and $\bar{s}$.}
	\KwResult{An approximate solution for \lcs.}
	
	Construct an $\sqrt{n} \times \sqrt{n}$ table $T$ with the following property:\\
	$T[i][j] := $ the number of occurrences of the character is which appeared the most in both $\block_i$ and $\barblock_j$\;
	Compute the length of the longest restricted common subsequence of $s$ and $\bar{s}$ using dynamic program described by Formula \eqref{eq:2}\;
	\caption{block-to-block Algorithm}
	\label{alg:3}
\end{algorithm}

Since the size of $\flcs$ is $\omegabar(n)$ and each string has $\sqrt n$ blocks, both $s$ and $\bar{s}$ contain at least $\omegabar(\sqrt{n})$ valuable blocks. In Lemma \ref{lem:block_match} we show that in the hard instances, the valuable blocks of $s$ and $\bar{s}$ can be perfectly matched. 



%In the next step, we divide every string into blocks of size $\sqrt{n}$. Let $\ell_i$ and $r_i$  be the starting and ending indices of the $i$'th block of $s$ and $s_{\ell_i,r_i}$ be the substring of $s$ containing only block $i$. 
 
%Now construct a bipartite graph $G(X,Y)$ as follows: vertices of $X$ refer to the block of $s$ and the vertices of $Y$ refer to the block of $\bar{s}$, and there is an edge between $x_i \in X$ and $y_j \in Y$, if $\llcs()

\begin{lemma}
	\label{lem:block_match}
	 Let $\flcs = \omegabar(n)$. Then, there exists two sequences $i_1 < i_2 < \ldots < i_{l}$ and $j_1 < j_2 < \ldots < j_{l}$ of indices such that $l = \omegabar(\sqrt n)$, and for every $k$, $\llcs(\block_{i_k},\barblock_{j_k})= \bar{\theta}({\sqrt{n})}.$ 
\end{lemma}
\begin{proof}
	Let $p_i$ and $q_i$ be the block number that the $i$'th symbol of  $\flcs$ belongs to in $s$ and $\bar{s}$, respectively, and let $U$ be a multi-set containing these pairs. We know both the sequences $p_1,p_2, \ldots, p_{|\flcs|}$ and $q_1,q_2, \ldots, q_{|\flcs|}$ are non-decreasing. Thus, if for some $j$, $(p_j,q_j) \neq (p_{j+1},q_{j+1})$, at least one of these two inequalities hold: $$p_{j+1} >p_j \qquad \mbox{ or }\qquad q_{j+1}>q_j.$$ As a result, total number of different pairs in $U$ is at most $2\sqrt{n} = \tildbar(\sqrt n).$	
	Since $|U| = \omegabar(n)$, we can find $\omegabar(\sqrt n)$ different pairs which appeared $\omegabar(\sqrt n)$ times in $U$. Let $P$ be the set of these pairs. Say pair $(p_i,q_i)$ collides pair $(p_j,q_j)$, if either $p_i = p_j$ or $q_i = q_j$. Since the size of each block in $s$ and $\bar{s}$ is $\sqrt n$ and each pair in $P$ is appeared $\omegabar(\sqrt n)$ times in $U$, no pair $(p_i,q_i)$ in $P$ can collide more than $\tildbar(1)$ other pairs in $P$. Otherwise, at least one of $\block_{p_i}$ or $\barblock_{q_i}$ must have size $\bar{\omega}(\sqrt n)$.
	Hence, $P$ contains at least $\omegabar(\sqrt{n})$ collision-free pairs, with each of them appeared $\omegabar(\sqrt{n})$ times in $U$. Each one of these pairs refers to a pair of blocks in $s$ and $\bar{s}$.
\end{proof}

\color{magenta}
Note that these blocks contribute $\omegabar(n)$ characters to $\llcs(s,\bar s)$. For each pair $(\block_{i_k},\barblock_{j_k})$ , let $f_k$ be the frequency of the character that is most appeared in both of these blocks. We know the length of the longest constrained common subsequence of $s$ and $\bar{s}$ is at least $\sum_i f_i$. Thus, Observation \ref{obs:7} holds.

\begin{observation}
	\label{obs:7}
	If there exists a constant $\epsilon>0$ such that $$\sum_{1 \leq i \leq l} f_i \geq n^{1/2+\epsilon},$$ then Algorithm \ref{alg:3} is a $\tildbar(n^{1/2-\epsilon})$ approximation of $\lcs$.
\end{observation}

As a consequence of Observation \ref{obs:7}, number of the indices $k$ such that $f_k = \omegabar(n^\epsilon)$ is $\tildo(\sqrt n)$, and  therefore, for $\omegabar(\sqrt n)$ of the blocks we have $f_k =  \tildbar(1)$.
These blocks contribute $\omegabar(n)$ characters to $\flcs$. Thus, we can restrict our attention only to the blocks with $f_k=\tildbar(1)$ and leave the rest of the blocks aside. 
 \color{black}
\begin{observation}
	\label{obs:10}
	We can assume w.l.o.g that in the hard instances, for every $k$, the frequency of each character in both $\block_{i_k}$ and $\barblock_{j_k}$ is $\tildbar(1)$.
\end{observation}

In the rest of this draft, we use $i_1,i_2,.\ldots,i_{l}$ and $j_1,j_2,\ldots,j_{l}$ to refer to the indices of these blocks in $s$ and $\bar{s}$. 
Now, we prune $s$ and $\bar{s}$ with the following operation on every block $\block_i$: for every character which is appeared more than once in $\block_i$, we select one of them uniformly at random and remove the rest. We claim that after pruning $s$ and $\bar{s}$, $\flcs$ is still $\omegabar(n)$. More precisely, we argue that for every $k$, $$\llcs(\block_{i_k},\barblock_{j_k}) = \omegabar(\sqrt n).$$ 

\begin{lemma}
	After pruning $s$ and $\bar{s}$, for every $k$ we have $\llcs(\block_{i_k},\barblock_{j_k}) = \omegabar(\sqrt n)$.
\end{lemma}
\begin{proof}
	Consider blocks $\block_{i_k}$ and $\barblock_{j_k}$.
	By Observation \ref{obs:10}, no character can have a frequency of $\omegabar(n^\epsilon)$ for a constant $\epsilon$ in both $\block_{i_k}$ and $\block_{j_k}$. Thus, for every character $c$, one of the following two cases can occur: 
	\begin{itemize}
		\item Frequency of  $c$ is $\tildbar(1)$ in both $\block_{i_k}$ and $\barblock_{j_k}$.
		\item Frequency of  $c$ is $\omegabar(n^\epsilon)$ in one of the blocks  $\block_{i_k},\barblock_{j_k}$ and $\tildbar(1)$ in the other.  
	\end{itemize}
	Consider $\llcs(\block_{i_k},\barblock_{j_k})$. Say a symbol  in $\llcs(\block_{i_k},\barblock_{j_k})$ is pruned, if at least one of its corresponding symbols in $\block_{i_k}$ or $\barblock_{j_k}$ is removed in the pruning phase.  For the first case, since the frequency of the symbol is $\tildbar(1)$ in both $\block_{i_k}$ and $\block_{j_k}$, the character is not pruned with probability $\omegabar(1)$. On the other hand, number of the characters of the second type in $\llcs(\block_{i_k},\barblock_{j_k})$ is at most $\tildbar(n^{1/2-\epsilon})$. Thus, $\omegabar(\sqrt n)$ of the characters in $\llcs(\block_{i_k},\barblock_{j_k})$ are of the first type, and since each one of these $\omegabar(\sqrt n)$ characters remain in $\flcs$ with probability $\omegabar(1)$, the expected size of $\llcs(\block_{i_k},\barblock_{j_k})$ is at least $\omegabar(\sqrt n)$.
\end{proof}


\begin{comment}
\begin{observation}
	Consider $x$ to be an optimal solution for $\mathsf{lcs}(s,\bar{s})$. Let $d_i$ be the smallest $j$ such that $x_j = x_{i+j}$. If the average value for $d_i$ is bounded by $\tildbar(n^{0.49})$, then Algorithm \ref{alg:3} is $\tildbar(n^{0.49})$ approximate.
\end{observation}
\end{comment}

%\begin{lemma}
%	Construct $s'$, $\bar{s}'$ from $s$ and $\bar{s}$ and I mentioned. If Algorithm \ref{alg:3} is $\Omega(n^{1/2-\epsilon})$ approximate, then $\mathsf{lcs}(s,\bar{s})$ and $\mathsf{lcs}(s',\bar{s}')$ are within a factor of $\tildbar(n^\epsilon)$.
%\end{lemma}


\begin{definition}
	String $s$ is a semi-permutation string, if it can be partitioned into $\sqrt n$ blocks, each of size $\omegabar(\sqrt n)$, such that each block is a permutation of the characters in $m$, except that some of the characters are missing in each permutation. In addition, if we select a random character and a random  block, this character is appeared in the block with probability $\omegabar(1)$.
\end{definition}

It is easy to observe that after pruning $s$ and $\bar{s}$, we are faced with two semi-permutations. Thus, finding $\flcs$ can be reduced to finding longest common subsequence of two strings which are semi-permutations. 

\begin{observation}
	\label{obs:semi}
	We can suppose w.l.o.g that both $s$ and $\bar{s}$ are semi-permutations.
\end{observation}

To summarize this section, regarding Observation \ref{obs:semi} and Lemma \ref{lem:block_match}, we can concentrate our attention to the instances where each of $s$ and $\bar{s}$ is a semi-permutation, and there are $l = \omegabar(\sqrt n)$ blocks in each string, say $i_1,i_2,.\ldots,i_{l}$ and $j_1,j_2,\ldots,j_{l}$ such that for every $k$, $\llcs(\block_{i_k}, \barblock_{j_k}) = \omegabar(\sqrt n)$. 


In the next section, we consider the case that each string is a semi-permutation.

%\color{red}Saeed: define the semi-permutation as follows: it is like a permutation with the exception that some of the characters are missing in every permutation. It is essential to have a restriction like this: if we select a random character and a random permutation, the character appears in that permutation with probability at least $\omegabar(1)$.\color{black}

==> permutation.tex <==
\section{Approximating Semi Permutation}

In this section, we consider the case that both $s$ and $\bar{s}$ are semi-permutations. By definition, each one of $s$ and $\bar{s}$ is a concatenation of $\sqrt n$ blocks, where each block is a permutation of a subset of the characters in $\Sigma$. Moreover, the probability that a random character appears in a random block is $\omegabar(1)$ and we have $m = \bar{\theta}(\sqrt n)$. For this case, we propose algorithm \ref{alg:4}. 

First, let us describe Algorithm \ref{alg:4} in details. This algorithm simply samples a random integer $r$ uniformly from $[1,\sqrt n]$ and then for every $i$, finds $q_i = \llcs(\block_i,\barblock_{(i+r) \mod \sqrt n})$. Note that $q_i$ can be found in time $\tildbar(\sqrt n)$, since $\block_i$ and $\barblock_{(i+r) \mod \sqrt n}$ contain $\tildbar(\sqrt n)$ matching pairs. Next, the algorithm selects one of $q_1q_2\ldots q_{\sqrt n-r}$ or $q_{\sqrt n-r+1}q_{\sqrt n-r+2}\ldots q_{\sqrt n}$ which is longer, as an approximation of $\flcs$. 

\begin{algorithm}[H]
	\KwData{
		$s$ and $\bar{s}$, both of which are complete permutations}
	\KwResult{An approximate solution for \lcs.}
	$r \leftarrow $a random integer number between $1$ and $\sqrt{n}$. \;
	\For{$i \in [1,\sqrt n]$ }{
		$q_i \leftarrow \llcs(\block_i,\barblock_{(i+r) \mod n})$
	}
	return $\arg \max\{|q_1q_2q_{\sqrt n-r}|,|q_{\sqrt n-r+1}q_{\sqrt n-r+2}\ldots q_{\sqrt n}|\}$
	\caption{Random selection}
	\label{alg:4}
\end{algorithm}

Throughout this section, we show that when both the strings are semi-permutations, Algorithm \ref{alg:4} returns a solution which is a $\bar{o}(\sqrt n)$ approximation of $\flcs$. We start by proving Observation \ref{obs:6}.

\begin{observation}
	\label{obs:6}
	If there exists a constant $\epsilon>0$ such that for every two randomly selected blocks $\block_i$ and $\barblock_j$,  $$\mathbb{E}[\llcs(\block_i, \barblock_j)] =  \omegabar(n^{\epsilon}),$$  then Algorithm \ref{alg:4} is a $\tildbar(n^{1/2-\epsilon})$ approximation for $\lcs$. 
\end{observation}

\begin{proof}
	Assume that there exists a constant $\epsilon>0$, where for every two randomly selected blocks of $s$ and $\bar{s}$, the expected size of the  longest common subsequence of the blocks is $\omegabar(n^\epsilon)$. Since $r$  is selected uniformly at random in Algorithm \ref{alg:4}, the expected size of each $q_i$ is $\omegabar(n^\epsilon)$. Thus, the expected size of the string $q_1q_2\ldots q_{\sqrt n}$ is $\omegabar(n^{1/2+\epsilon})$. On the other hand, 
	$$
	\max\{|q_1q_2q_{\sqrt n-r}|,|q_{\sqrt n-r+1}q_{\sqrt n-r+2}\ldots q_{\sqrt n}|\} \geq |q_1q_2\ldots q_{\sqrt n}|/2,
	$$
	which means that the solution returned by Algorithm \ref{alg:4} is a $\tildbar(n^{1/2-\epsilon}) = \bar{o}(\sqrt n)$ approximation. 
	
\end{proof}

Our strategy to deal with the case of semi-permutations is to prove that the condition of Observation \ref{obs:6} is satisfied for any two semi-permutations. To show this, we first refine  $s$ and $\bar s$ and convert them to complete permutations. In the following, we define the refinement process. For brevity, we only describe the process for $s$. The same process must be applied to the blocks in $\bar s$. 

\textbf{Refining string $s$}: The refinement process of string $s$ is described in Algorithm \ref{refine}. This algorithm, takes $s$ as input and updates each block $\block_i$ of $s$ as follows: first, it chooses $d\log n$ blocks of $s$ uniformly at random, where $d$ is a constant to be determined later. Next, it observes these blocks one by one, and  for each block $b$, appends the characters in $b$ that are not in $\block_i$ to the end of $\block_i$, with the same order  as they are appeared in $b$. Finally, there might still some characters in $\Sigma$ that are not appeared in $\block_i$. If so, we add them to the end of $\block_i$ arbitrarily. 

\begin{algorithm}[H]
	\KwData{
		$s = \block_1\block_2\ldots \block_k$: a semi-permutation.}
	\KwResult{A refined string $s'$ which is a complete permutation.}
	
	\For{$i \in [1,k]$ }{
		$b'_i \leftarrow \block_i$ \;
		$B:$ A set of $d\log n$ blocks of $s$ selected uniformly at random\;
		\For{each $b \in B$}{
			$r = $ maximal substring of $b$ consisted only from the characters in $\Sigma \setminus b'_i$ \;
			$b'_i \leftarrow b'_i + r$\;
		}
		\If {$\block_i$ is not a permutation}{
			Add the characters in $\Sigma \setminus b'_i$ with an arbitrary order to the end of $b'_i$
		}
	}
	return $s' = b'_1b'_2\ldots b'_k$
	\caption{Refining $s$}
	\label{refine}
\end{algorithm}

\vspace{0.5cm}
After refining $s$, each block $\block_i$ of $s$ is consisted of three parts: the original part, the part that is appended to $\block_i$ with respect to the other blocks, and the part that includes the characters that are added to $\block_i$ in an arbitrary order. We denote these three parts by $o_i,w_i,$ and $a_i$, respectively. 
By definition of semi-permutation, each character is appeared in each of the randomly selected blocks with probability $\omegabar(1)$, which means there exists a constant $z$ that the probability is more than $z$.
In Observation \ref{obs:numblock} we show that by choosing $d = 1/(2\log (1-z))$, the expected size of  $a_i$ is $\tildbar(1)$ for each block $\block_i$. 



\begin{observation}
	\label{obs:numblock}
	If $d = 1/(2\log (1-z))$, then the expected size of $a_i$ for each block $\block_i$ is $\tildbar(1)$. 
\end{observation}
\begin{proof}
	Let $p_c$ be the probability that after appending the extra characters in $d\log n$ randomly selected blocks, $\block_i$ does not contain character $c$. By definition of semi-permutation, $c$ is appeared in each of the randomly selected blocks with probability at least $z$. Hence, after $d\log n$ steps, we have 
	$$
	p_c \leq (1-z)^{d\log n} = n^{d\log(1-z)}.
	$$
	On the other hand, we know $m = \bar{\theta}(\sqrt n)$, meaning that there is a constant $z'$, such that the number of characters in $\Sigma$ is at most $z'\sqrt n$. Thus, we have 
	\begin{align*}
	\mathbb{E}(|a_i|) &= \sum_c p_c \\
	&\leq \sum_c 	n^{d\log(1-z)} \\
	&\leq z'n^{1/2} n^{d\log(1-z)}\\
	&= z' n^{1/2-d\log(1-z)}.
	\end{align*}
	If we set $d= 1/(2\log (1-z))$ we have $\mathbb{E}(|a_i|) \leq z' = \tildbar(1)$.   
\end{proof}

Since $s$ initially was a semi-permutation, after refining $s$, for every character $c$ and a randomly selected block $\block_i$, the probability that $c \in o_i$ is $\tildbar(1)$.
Now, let $e$ be the expected size of the longest common subsequence of two randomly selected blocks of $s$ and $\bar{s}$, before the refining process. After refining $s$ and $\bar{s}$, we know that each block of $s$ and $\bar{s}$ is a concatenation of at most $d\log n$ strings, each of which is a substring of a randomly selected block, plus a string of size $\tildbar(1)$.  According to this, we can conclude that after the refinement process, the expected size of the longest common subsequence of two randomly selected blocks is $\tildbar((d\log n)^2 e) = \tildbar(e)$. Thus, Observation \ref{obs:lcsblock} holds.

\begin{observation}
	\label{obs:lcsblock}
Let $e$ be the expected size of two randomly selected blocks of $s$ and $\bar{s}$, before the refining process. After refining $s$ and $\bar{s}$, the expected size of the longest common subsequence of two randomly selected blocks is still $\tildbar(e)$.
\end{observation}

After refining $s$ and $\bar{s}$, we are faced with two complete permutations: two strings, with each of them consisting $\sqrt n$ blocks, where each block is a permutation of the characters in $\Sigma$.  
Recall that the size of the solution is $\omegabar(n)$. In the rest of this section, we show that the condition in Observation \ref{obs:6} holds for any two complete permutation strings. To show this we use two well-known theorems, one in the context of order theory and the other in graph theory. 

\begin{theorem}[Dilworth-restated for the case of string matching]
	\label{dilworth}
	Given two strings $\pi$ and $\bar{\pi}$, each of which is a permutation of $[m]$\footnote{By $[x]$, we mean $\{1,2,\ldots,x\}$.}. If $\llcs(\pi,\bar{\pi}) = x$, then $\bar{\pi}$ can be decomposed into $x$ substrings, such that the characters in each of these strings are appeared exactly in the reverse order that are appeared in $\pi$, i.e., the longest common subsequence of each of these substrings and $\pi$ is $1$.
\end{theorem}

\begin{theorem}[Turan]
	\label{turan}
	Any triangle-free graph of size $n$ has at most $n^2/4$ vertices.
\end{theorem}

First, we use Dilworth theorem to prove Lemma \ref{lem:3block}. 
\begin{lemma}
	\label{lem:3block}
	Let $\pi_1, \pi_2, \pi_3$ be three permutations of $[m]$. Then, we have 
	$$
	\llcs(\pi_1,\pi_2) \cdot \llcs(\pi_2,\pi_3) \cdot \llcs(\pi_3,\pi_1) \geq m.
	$$
\end{lemma}

\begin{proof}
	Consider $\pi_1$ and $\pi_2$ and suppose that $\llcs(\pi_1,\pi_2) = x$ and $\llcs(\pi_1,\pi_3)=y$. According to Theorem \ref{dilworth}, $\pi_2$ and $\pi_3$ can be respectively decomposed into $x$ and $y$ substrings, such that the characters in each of these substrings are appeared in the reverse order as appeared in $\pi_1$. On the other hand, by the Pigeonhole principle, at least one of the substrings of $\pi_1$ and one of the substrings of $\pi_2$ have $m/xy$ characters in common. Since these characters are appeared in the same order in both of these substrings, the longest common subsequence of these two substrings is at least $m/xy$. Thus we have
	\begin{align*}
	\llcs(\pi_1,\pi_2) \cdot \llcs(\pi_2,\pi_3) \cdot \llcs(\pi_3,\pi_1) &\geq  x \cdot y \cdot m/xy \\
	&= m
	\end{align*}	
\end{proof}

Recall that in the previous section, we showed that $s$ and $\bar{s}$ contain $l = \omega(\sqrt n)$ pairs of blocks, $(\block_{i_1},\barblock_{i_1}),(\block_{i_2},\barblock_{i_2}),\ldots,(\block_{i_l},\barblock_{i_l})$, such that both $i_k$'s and $j_k$'s are increasing and for every $k$, $\llcs(\block_{i_k},\barblock_{i_k}) = \omegabar(\sqrt n)$. We use this fact along with Theorem \ref{turan} to lower-bound the expected size of the longest common subsequence of two randomly selected blocks of $s$ and $\bar{s}$. \textcolor{magenta}{A little imprecise}

\begin{definition}
	Consider a Graph $G(V,E)$ where each $v_k \in V$ corresponds to block pair  $(\block_{i_k},\block_{j_k})$ and there is an edge between $v_{k}$ and $v_{k'}$, if at least one of the following two conditions hold:
	\begin{itemize}
		\item $\llcs(\block_{i_k},\barblock_{j_k'}) = \omegabar(n^{1/6})$.
		\item $\llcs(\block_{i_k'},\barblock_{j_k}) = \omegabar(n^{1/6})$.
	\end{itemize}
\end{definition}
Note that by Lemma \ref{lem:3block}, For every three vertices $v_k,v_{k'},v_{k''}$, at least one of the edges $(v_k,v_{k'}),(v_{k'},v_{k''})$, and $(v_{k},v_{k''})$ is in $E$, and hence the complement graph $\bar{G}$ is triangle-free, and by Theorem \ref{turan}, $\bar{G}$ contains at most $n/4$ edges. Thus, $|E| \geq (n-2 \sqrt n)/2 = \omegabar(n)$ edges, which means 
\begin{align*}
\sum_{k,k'} \llcs(\block_{i_k},\block_{j_{k'}}) \in \omegabar(n \cdot n^{1/6} + \sqrt n \cdot \sqrt n) = \omegabar(n^{7/6}).  
\end{align*}
Since there are $n$ pairs of blocks, the expected size of the longest common subsequence of two randomly selected block is $\omegabar(n^{1/6})$. According to Observation \ref{obs:lcsblock}, the same holds for $s$ and $\bar{s}$, before the refinement procedure: the expected size of the longest common subsequence of two randomly selected blocks is at least $\omegabar(n^{1/6})$. Considering Observation \ref{obs:numblock}, this means that Algorithm \ref{alg:4} returns a $\bar{o}(\sqrt n)$ approximation for the longest common subsequence of two semi-permutations. 

\begin{observation}
	\label{obs:comp}
	For two semi-permutations $s$ and $\bar{s}$, Algorithm \ref{alg:4} returns a $\bar{o}(\sqrt{n})$ approximation of $\flcs$. 
\end{observation}




%On the other hand, we know that the longest common subsequence of two randomly selected blocks of $s$ and $\bar{s}$ after refining is $\omegabar(n^{1/6})$, which means $e = \omegabar(n^{1/6})$.  Note that the structure of Algorithm \ref{alg:4} is independent of the size of each block, that is, Observation \ref{obs:6} holds, even if two strings $s$ and $\bar{s}$ are semi-permutations. Hence, Observation \ref{obs:final} holds.


% which means Algorithm \ref{alg:4} returns a solution of size  $\omegabar(n^{1/2+1/6})$ approximation of $\flcs$. However, some of the characters in the solution returned by Algorithm \ref{alg:4} might belong to $w_i$ or $a_i$ for some $i$. In Observation \ref{obs:bound} we bound the expected number of the characters in $\flcs$ that belong to $o_i$. 





%\begin{observation}
%	\label{obs:bound}
%	Let $s$ and $\bar{s}$ be two complete permutation obtained from refining two semi-permutations and let $r$ be the solution returned by Algorithm \ref{alg:4}. For each symbol in $r$, we label it with $o$, if its corresponding symbols in $s$ and $\bar{s}$ belong to the original part of the blocks. Then, the expected number of the symbols in $\flcs$ label with $o$ is $\tildbar(n)$.
%\end{observation}




%Now, consider $\flcs$ after refining $s$ and $\bar{s}$.   Say a symbol in $\flcs$ is original, if \textcolor{magenta}{to be continued...}


\begin{figure}
	\centerline{\includegraphics[scale=0.8]{figs/flowchart3}}
\end{figure}


%\begin{figure}
%	\centerline{\includegraphics[scale=0.8]{figs/pruning}}
%\end{figure}



==> windows.tex <==
\begin{figure}[h!]

\begin{center}
\begin{tikzpicture}[scale=0.96, transform shape]

%\draw (0,0) -- (15.4,0) -- (15.4,0.5) -- (0,0.5) -- (0,0);
%\node[text width=3cm] at (9,0.2) 
%{$a$};

%\node[text width=3cm, rotate = 90] at (-0.5,2.6) 
%{    \Huge$\overbrace{\hspace{3.9cm}}$   };
%\node[text width=3cm, rotate = 90] at (-1.3,3.2) 
%{  $\log n +1$ rounds  };

%\node[text width=3cm] at (3.9,5.2) 
%{    \huge$\overbrace{\hspace{3.0cm}}$   };



\node[text width=3cm, rotate = 90] at (7.72,4.1) 
{  \huge  $\ldots$   };

\draw (-0.1,1.1) -- (15.5,1.1) -- (15.5,1.8) -- (-0.1,1.8) -- (-0.1,1.1);
\draw[dashed] (0,1.2) -- (0.4,1.2) -- (0.4,1.7) -- (0,1.7) -- (0,1.2);
\draw[dashed] (0.5,1.2) -- (0.9,1.2) -- (0.9,1.7) -- (0.5,1.7) -- (0.5,1.2);
\draw[dashed] (1,1.2) -- (1.4,1.2) -- (1.4,1.7) -- (1,1.7) -- (1,1.2);
\draw[dashed] (1.5,1.2) -- (1.9,1.2) -- (1.9,1.7) -- (1.5,1.7) -- (1.5,1.2);
\draw[dashed] (2,1.2) -- (2.4,1.2) -- (2.4,1.7) -- (2,1.7) -- (2,1.2);
\draw[dashed] (2.5,1.2) -- (2.9,1.2) -- (2.9,1.7) -- (2.5,1.7) -- (2.5,1.2);
\draw[dashed] (3,1.2) -- (3.4,1.2) -- (3.4,1.7) -- (3,1.7) -- (3,1.2);
\draw[dashed] (3.5,1.2) -- (3.9,1.2) -- (3.9,1.7) -- (3.5,1.7) -- (3.5,1.2);
\draw[dashed] (4,1.2) -- (4.4,1.2) -- (4.4,1.7) -- (4,1.7) -- (4,1.2);
\draw[dashed] (4.5,1.2) -- (4.9,1.2) -- (4.9,1.7) -- (4.5,1.7) -- (4.5,1.2);
\draw[dashed] (5,1.2) -- (5.4,1.2) -- (5.4,1.7) -- (5,1.7) -- (5,1.2);
\draw[dashed] (5.5,1.2) -- (5.9,1.2) -- (5.9,1.7) -- (5.5,1.7) -- (5.5,1.2);
\draw[dashed] (6,1.2) -- (6.4,1.2) -- (6.4,1.7) -- (6,1.7) -- (6,1.2);
\draw[dashed] (6.5,1.2) -- (6.9,1.2) -- (6.9,1.7) -- (6.5,1.7) -- (6.5,1.2);



\draw[dashed] (8.5,1.2) -- (8.9,1.2) -- (8.9,1.7) -- (8.5,1.7) -- (8.5,1.2);
\draw[dashed] (9,1.2) -- (9.4,1.2) -- (9.4,1.7) -- (9,1.7) -- (9,1.2);
\draw[dashed] (9.5,1.2) -- (9.9,1.2) -- (9.9,1.7) -- (9.5,1.7) -- (9.5,1.2);
\draw[dashed] (10,1.2) -- (10.4,1.2) -- (10.4,1.7) -- (10,1.7) -- (10,1.2);
\draw[dashed] (10.5,1.2) -- (10.9,1.2) -- (10.9,1.7) -- (10.5,1.7) -- (10.5,1.2);
\draw[dashed] (11,1.2) -- (11.4,1.2) -- (11.4,1.7) -- (11,1.7) -- (11,1.2);
\draw[dashed] (11.5,1.2) -- (11.9,1.2) -- (11.9,1.7) -- (11.5,1.7) -- (11.5,1.2);
\draw[dashed] (12,1.2) -- (12.4,1.2) -- (12.4,1.7) -- (12,1.7) -- (12,1.2);
\draw[dashed] (12.5,1.2) -- (12.9,1.2) -- (12.9,1.7) -- (12.5,1.7) -- (12.5,1.2);
\draw[dashed] (13,1.2) -- (13.4,1.2) -- (13.4,1.7) -- (13,1.7) -- (13,1.2);
\draw[dashed] (13.5,1.2) -- (13.9,1.2) -- (13.9,1.7) -- (13.5,1.7) -- (13.5,1.2);
\draw[dashed] (14,1.2) -- (14.4,1.2) -- (14.4,1.7) -- (14,1.7) -- (14,1.2);
\draw[dashed] (14.5,1.2) -- (14.9,1.2) -- (14.9,1.7) -- (14.5,1.7) -- (14.5,1.2);
\draw[dashed] (15,1.2) -- (15.4,1.2) -- (15.4,1.7) -- (15,1.7) -- (15,1.2);
%\draw[dashed] (6.2,1.2) -- (9.2,1.2) -- (9.2,1.7) -- (6.2,1.7) -- (6.2,1.2);
\node[text width=3cm] at (8.8,1.4) 
{   \huge $\ldots$   };

\node[text width=3cm] at (17.1,1.4) 
{   round $\log n +1$  };

%\draw[dashed] (9.3,1.2) -- (12.3,1.2) -- (12.3,1.7) -- (9.3,1.7) -- (9.3,1.2);
%\draw[dashed] (12.4,1.2) -- (15.4,1.2) -- (15.4,1.7) -- (12.4,1.7) -- (12.4,1.2);

%\draw[dashed] (0.6,2) -- (3.6,2) -- (3.6,2.5) -- (0.6,2.5) -- (0.6,2);
%\draw[dashed] (3.7,2) -- (6.7,2) -- (6.7,2.5) -- (3.7,2.5) -- (3.7,2);
%\draw[dashed] (6.8,2) -- (9.8,2) -- (9.8,2.5) -- (6.8,2.5) -- (6.8,2);

\draw (-0.1,1.9) -- (15.5,1.9) -- (15.5,2.6) -- (-0.1,2.6) -- (-0.1,1.9);
\draw[dashed] (0,2) -- (0.9,2) -- (0.9,2.5) -- (0,2.5) -- (0,2);
\draw[dashed] (1,2) -- (1.9,2) -- (1.9,2.5) -- (1,2.5) -- (1,2);
\draw[dashed] (2,2) -- (2.9,2) -- (2.9,2.5) -- (2,2.5) -- (2,2);
\draw[dashed] (3,2) -- (3.9,2) -- (3.9,2.5) -- (3,2.5) -- (3,2);
\draw[dashed] (4,2) -- (4.9,2) -- (4.9,2.5) -- (4,2.5) -- (4,2);
\draw[dashed] (5,2) -- (5.9,2) -- (5.9,2.5) -- (5,2.5) -- (5,2);
\draw[dashed] (6,2) -- (6.9,2) -- (6.9,2.5) -- (6,2.5) -- (6,2);


\draw[dashed] (8.5,2) -- (9.4,2) -- (9.4,2.5) -- (8.5,2.5) -- (8.5,2);
\draw[dashed] (9.5,2) -- (10.4,2) -- (10.4,2.5) -- (9.5,2.5) -- (9.5,2);
\draw[dashed] (10.5,2) -- (11.4,2) -- (11.4,2.5) -- (10.5,2.5) -- (10.5,2);
\draw[dashed] (11.5,2) -- (12.4,2) -- (12.4,2.5) -- (11.5,2.5) -- (11.5,2);
\draw[dashed] (12.5,2) -- (13.4,2) -- (13.4,2.5) -- (12.5,2.5) -- (12.5,2);
\draw[dashed] (13.5,2) -- (14.4,2) -- (14.4,2.5) -- (13.5,2.5) -- (13.5,2);
\draw[dashed] (14.5,2) -- (15.4,2) -- (15.4,2.5) -- (14.5,2.5) -- (14.5,2);

\node[text width=3cm] at (8.8,2.2) 
{   \huge $\ldots$   };
%\draw[dashed] (9.9,2) -- (12.9,2) -- (12.9,2.5) -- (9.9,2.5) -- (9.9,2);
\node[text width=3cm] at (17.1,2.2) 
{   round $\log n$  };


%\draw[dashed] (1.2,2.8) -- (4.2,2.8) -- (4.2,3.3) -- (1.2,3.3) -- (1.2,2.8);
%\draw[dashed] (4.3,2.8) -- (7.3,2.8) -- (7.3,3.3) -- (4.3,3.3) -- (4.3,2.8);
%\draw[dashed] (7.4,2.8) -- (10.4,2.8) -- (10.4,3.3) -- (7.4,3.3) -- (7.4,2.8);
%\node[text width=3cm] at (10.0,3.0) 
%{   \huge $\ldots$   };
%\draw[dashed] (10.5,2.8) -- (13.5,2.8) -- (13.5,3.3) -- (10.5,3.3) -- (10.5,2.8);

\draw (-0.1,3.5) -- (15.5,3.5) -- (15.5,4.2) -- (-0.1,4.2) -- (-0.1,3.5);
\draw[dashed] (0,3.6) -- (7.6,3.6) -- (7.6,4.1) -- (0,4.1) -- (0,3.6);
%\draw[dashed] (1.8,3.6) -- (4.8,3.6) -- (4.8,4.1) -- (1.8,4.1) -- (1.8,3.6);
%\draw[dashed] (4.9,3.6) -- (7.9,3.6) -- (7.9,4.1) -- (4.9,4.1) -- (4.9,3.6);
%\draw[dashed] (8.0,3.6) -- (11.0,3.6) -- (11.0,4.1) -- (8.0,4.1) -- (8.0,3.6);
\draw[dashed] (7.8,3.6) -- (15.4,3.6) -- (15.4,4.1) -- (7.8,4.1) -- (7.8,3.6);
%\draw[dashed] (11.1,3.6) -- (14.1,3.6) -- (14.1,4.1) -- (11.1,4.1) -- (11.1,3.6);

\node[text width=3cm] at (17.1,3.8) 
{   round $2$  };

\draw (-0.1,4.3) -- (15.5,4.3) -- (15.5,5) -- (-0.1,5) -- (-0.1,4.3);
\draw[dashed] (0,4.4) -- (15.4,4.4) -- (15.4,4.9) -- (0,4.9) -- (0,4.4);
\node[text width=3cm] at (17.1,4.6) 
{   round $1$  };

\node[text width=3cm] at (1.42,5.3) 
{   $1$   };
\node[text width=3cm] at (16.62,5.3) 
{   $n$   };
%\draw[dashed] (2.4,4.4) -- (5.4,4.4) -- (5.4,4.9) -- (2.4,4.9) -- (2.4,4.4);
%\draw[dashed] (5.5,4.4) -- (8.5,4.4) -- (8.5,4.9) -- (5.5,4.9) -- (5.5,4.4);
%\draw[dashed] (8.6,4.4) -- (11.6,4.4) -- (11.6,4.9) -- (8.6,4.9) -- (8.6,4.4);
%\node[text width=3cm] at (11.2,4.6) 
%{   \huge $\ldots$   };
%\draw[dashed] (11.7,4.4) -- (14.7,4.4) -- (14.7,4.9) -- (11.7,4.9) -- (11.7,4.4);




%\node [draw,rounded corners,minimum height=5cm,minimum width=4cm] (node1) {};
%\node [anchor=north west,minimum width=10cm] at (-3.6,1) {\fbox{\hspace{1cm}$w_1$\hspace{1cm}}};
%\node [anchor=north west,minimum width=10cm] at (-0.9,1) {\fbox{\hspace{1cm}$$\hspace{1cm}}};
%\node [anchor=north west,minimum width=10cm] at (1.8,1) {\fbox{\hspace{1cm}$\ldots$\hspace{1cm}}};
%\node [anchor=north west,minimum width=10cm] at (4.5,1) {\fbox{\hspace{1cm}$$\hspace{1cm}}};
%\node [anchor=north west,minimum width=10cm] at (7.2,1) {\fbox{\hspace{1cm}$$\hspace{1cm}}};
%\node [anchor=north west,minimum width=10cm] at (0,0) {\fbox{\hspace{6.4cm}$s_1$\hspace{6.4cm}}};
% {\fbox{\hspace{6.4cm}$s_1$\hspace{6.4cm}}};

%\node [anchor=south west] at (node1.north west) {\fbox{Case: anchor is SW}};
%\node [anchor=south east] at (node1.north west) {\fbox{Case: anchor is SE}};
%\node [anchor=north east] at (node1.north west) {\fbox{Case: anchor is NE}};
%\foreach \myanchor in {north west}
%{ 
%	\node[fill,circle,inner sep=1pt,outer sep=1ex,anchor=\myanchor] at (node1.north west){};
%}
\end{tikzpicture}
\end{center}
\caption{In every round $s+1$, $b$ is split into $2^s$ intervals of size $2^{\log n - s}$.}\label{figs:bs}
\end{figure}
